Measure Before You Manage: Evaluating Agent Working Memory in Coding Agents

Agent working memory is heterogeneous. Objects such as instructions, artifacts, tool outputs, and agent-generated state play different semantic roles and exhibit different size, retention, and representation profiles. Recent work has begun to explore memory-management mechanisms that account for such heterogeneity. This work focuses on semantic heterogeneity and studies how it should shape the management and evaluation of working memory in coding agents. Across 55 archived coding-agent trajectories, we find that semantically different working-memory objects exhibit distinct retention and compression behavior. This heterogeneity motivates semantically informed memory management. We study two semantically informed strategies: an object-aware compression policy and a retrieval-based policy. Their evaluation shows that calibration gains may not transfer to held-out tasks, and that equal token budgets do not imply equal delivered context or management cost. A real-system replay further exposes serving limits that nominal budgets alone do not capture. Together, these results show why semantic structure matters for agent working memory and why evaluating memory-management strategies requires more than a nominal token budget. We organize these lessons into four levels: stored state, delivered context, management work, and task or process outcome.

==> generated/app_block_ledger.tex <==
% Generated from saved records by analysis/build_appendix_evidence.py.
11870 & Complete & 3037 & 21.7 & -- \\
12481 & OA exhaustion & 1887 & 15.0 & -- \\
13146 & Complete & 2709 & 19.8 & -- \\
13437 & OA exhaustion & 993 & 15.0 & -- \\
13647 & Floor rule & 1438 & 26.1 & 16 \\
13773 & Floor rule & 1156 & 19.2 & 9 \\
14817 & Floor rule & 1517 & 19.2 & 3 \\
15609 & Floor rule & 1002 & 15.0 & 1 \\
16106 & Complete & 2849 & 28.4 & -- \\
16281 & Complete & 3689 & 25.2 & -- \\
17022 & Complete & 3069 & 15.0 & -- \\
17139 & Floor rule & 1332 & 60.2 & 2 \\
18057 & Floor rule & 1892 & 15.0 & 32 \\
18189 & Floor rule & 986 & 15.9 & 36 \\
18835 & Floor rule & 808 & 33.6 & 20 \\
19487 & Floor rule & 999 & 24.8 & 78 \\
20154 & Complete & 1682 & 17.2 & -- \\
20442 & Floor rule & 1034 & 24.2 & 68 \\
21055 & Floor rule & 1036 & 26.7 & 2 \\
21627 & Complete & 3494 & 15.0 & -- \\
22840 & OA exhaustion & 3458 & 44.3 & -- \\
23262 & Complete & 2172 & 36.6 & -- \\
24152 & Floor rule & 1222 & 76.7 & 12 \\
24213 & Floor rule & 926 & 39.4 & 12 \\


==> generated/app_h6_calibration.tex <==
% Generated from saved records by analysis/build_appendix_evidence.py.
sympy\_\_sympy-12481 & 2 & 1.5 & 0.5 & 1 \\
sympy\_\_sympy-13647 & 0 & 3 & 0 & 0 \\
sympy\_\_sympy-13773 & 1 & 0 & 1 & 0 \\
sympy\_\_sympy-14817 & 2 & 2 & 1 & 0 \\
sympy\_\_sympy-15609 & 1 & 0 & 0 & 0 \\
sympy\_\_sympy-17022 & 4 & 4 & 2 & 0.5 \\
sympy\_\_sympy-17139 & 0 & 0 & 1 & 1 \\
sympy\_\_sympy-18189 & 0 & 3 & 2 & 0 \\
sympy\_\_sympy-19487 & 2 & 0 & 0 & 0 \\
sympy\_\_sympy-20154 & 5.5 & 5.5 & 3 & 0 \\
sympy\_\_sympy-20442 & 6 & 6 & 2 & 0 \\
sympy\_\_sympy-21055 & 3.5 & 2.5 & 2.5 & 1.5 \\
sympy\_\_sympy-23262 & 0 & 0 & 0.5 & 0.5 \\
sympy\_\_sympy-24152 & 0 & 0 & 0 & 0 \\
sympy\_\_sympy-24213 & 2 & 0 & 0 & 0 \\


==> generated/app_h6_heldout.tex <==
% Generated from saved records by analysis/build_appendix_evidence.py.
mwaskom\_\_seaborn-3010 & 2 & 1 & 2 & 2 \\
mwaskom\_\_seaborn-3190 & 0 & 0 & 1 & 0 \\
psf\_\_requests-3362 & 0 & 8 & 1 & 0 \\
pylint-dev\_\_pylint-5859 & 1 & 0 & 2 & 0 \\
pylint-dev\_\_pylint-7228 & 0 & 0 & 1 & 0 \\
pytest-dev\_\_pytest-11148 & 0 & 5 & 0 & 0 \\
pytest-dev\_\_pytest-9359 & 5 & 5 & 5 & 2 \\
sphinx-doc\_\_sphinx-10325 & 0 & 0 & 0 & 0 \\

